A Cyclic Approach to the Annular Temperley-Lieb Category

In 2000, Jones found two copies of the cyclic category in the annular Temperley-Lieb category ATL. We give an abstract presentation of ATL to discuss how these two copies of the cyclic category generate ATL together with the coupling constants and the coupling relations. We then discuss modules over the annular category and homologies of such modules, the latter of which arises from the cyclic viewpoint.

==> pictures/BeamerTikzStyles.tex <==
\tikzstyle{shaded}=[fill=red!10!blue!20!gray!30!white]
\tikzstyle{shaded line}=[double=red!10!blue!20!gray!30!white, double distance=1.5mm, draw=black]
\tikzstyle{unshaded}=[fill=white]
\tikzstyle{unshaded line}=[double=white, double distance=1.5mm, draw=black]
\tikzstyle{Tbox}=[circle, draw, thick, fill=white, opaque,]
\tikzstyle{empty box}=[circle, draw, thick, fill=white, opaque, inner sep=2mm]
\tikzstyle{background rectangle}= [fill=red!10!blue!20!gray!40!white,rounded corners=2mm] 
\tikzstyle{on}=[very thick, red!50!blue!50!black]
\tikzstyle{off}=[gray]

%These are for resizing a family of drawings at the same time
\tikzstyle{traces}=[scale=.2, inner sep=1mm]
\tikzstyle{quadratic}=[scale=.4, inner sep=1mm, baseline]
\tikzstyle{annular}=[scale=.6, inner sep=1mm, baseline]
\tikzstyle{rectangular}=[scale=.6, inner sep=1mm, baseline]
\tikzstyle{make triple edge size}= [scale=.4, inner sep=1mm,baseline] 
\tikzstyle{icosahedron network}=[scale=.3, inner sep=1mm, baseline]
\tikzstyle{ATLsix}=[scale=.25, baseline]
\tikzstyle{TL12}=[scale=.15,baseline]
\tikzstyle{PAdefn}=[scale=.5,baseline]
\tikzstyle{TLEG}=[scale=.5,baseline]

==> pictures/atangle.tex <==
%%% a_1
\begin{tikzpicture}[annular]
%CIRCLES AND OUTER STAR
	\clip (0,0) circle (2cm);
	\draw[ultra thick] (0,0) circle (2cm);	
	\node at (180:1.80cm)  {$*$};
% THROUGH STRINGS
	\filldraw[shaded] (90:4cm)--(0,0)--(270:4cm) -- (0:4cm);	
	\draw[ultra thick] (0,0) circle (2cm);
	
\end{tikzpicture}

==> pictures/loop.tex <==
\begin{tikzpicture}[annular]
%CIRCLES AND OUTER STAR
	\clip (0,0) circle (2cm);
	\draw[ultra thick] (0,0) circle (2cm);	
	\node at (180:1.80cm) [right] {$*$};

	\filldraw[shaded] (0,0) circle (1cm);

%	\node at (T.120) [above] {$*$};		
\end{tikzpicture}
